UST: Unifying Spatio-Temporal Context for Trajectory Prediction in Autonomous Driving

Trajectory prediction has always been a challenging problem for autonomous driving, since it needs to infer the latent intention from the behaviors and interactions from traffic participants. This problem is intrinsically hard, because each participant may behave differently under different environments and interactions. This key is to effectively model the interlaced influence from both spatial context and temporal context. Existing work usually encodes these two types of context separately, which would lead to inferior modeling of the scenarios. In this paper, we first propose a unified approach to treat time and space dimensions equally for modeling spatio-temporal context. The proposed module is simple and easy to implement within several lines of codes. In contrast to existing methods which heavily rely on recurrent neural network for temporal context and hand-crafted structure for spatial context, our method could automatically partition the spatio-temporal space to adapt the data. Lastly, we test our proposed framework on two recently proposed trajectory prediction dataset ApolloScape and Argoverse. We show that the proposed method substantially outperforms the previous state-of-the-art methods while maintaining its simplicity. These encouraging results further validate the superiority of our approach.

==> content/__latexindent_temp.tex <==

\subsection{Results}
We compare our proposed method with several state-of-the-art algorithms and baseline models in this section.

\begin{table*}[!bt]
    % \tiny
    % \setlength{\tabcolsep}{0pt}
    % \centering
%			\begin{tabular}{+p{3cm}<{\centering}^c|^c^c^c^c}
%			\begin{minipage}{\textwidth}
    \begin{tabular}{@{}
        +m{1.0in}<{\centering}
        Ym{0.6in}<{\centering}Ym{0.6in}<{\centering}
        Ym{0.6in}<{\centering}Ym{0.6in}<{\centering}|Ym{0.6in}<{\centering}
        Ym{0.5in}<{\centering}Ym{0.5in}<{\centering}Ym{0.5in}<{\centering}%Ym{0.4in}<{\centering}
        @{}}
        \toprule
        & \multicolumn{3}{c} {(a) ADE}  & \multicolumn{5}{c}{(b) FDE }  \\
        % \cline{ 2-5 }\cline{ 6\quad-10 }
        % \noalign{\smallskip} 
        % \rowstyle{\tiny}
         & vehicles & pedestrians & bicycles & weighted & vehicles & pedestrians & bicycles & weighted \\
        \midrule{}
        %\multirow{8}{*}{$\epsilon=0.0$} 
        StarNet\cite{zhu2019starnet}                    &      2.38      &      0.78      &      1.86      &   1.34   &      4.28       &      1.51       &       3.46  &   2.49      \\
        TrafficPredict\cite{ma2019trafficpredict}                         &      7.94      &      7.18      &      12.88      &      8.58 &      12.77       &      11.12       &      22.79   &   24.22       \\
        LSTM  &      2.88      &      0.94      &      2.09      &    1.58   &      5.25       &      1.84       &      3.87    &  2.97       \\
        CV  &      2.59      &      0.81      &      2.17      &      1.47   &      4.64       &      1.58       &      4.02      &  2.73  \\
        \pmethodb                            &      \textbf{2.10}      &      \textbf{0.75}      &      \textbf{1.77}      &      \textbf{1.24}     &      \textbf{3.65}      &       \textbf{1.44}        &       \textbf{3.14}    &     \textbf{2.25}       \\
        \bottomrule
        %\protect\footnotemark
    \end{tabular}
    \caption{Performance on ApolloScape trajectory dataset. All result are recorded from ApolloScape public leaderboard. Our method is $1st$ rank currently. (a) shows the average distance error (ADE) of different algorithms on diverse traffic-agents. (b) shows the final distance error (FDE) in 3 second.}
%			\end{minipage}
\end{table*}\label{tab:apollo}
\paragraph{ApolloScape}
State-of-the-art algorithms on ApolloScape and baseline models are shown as follows.
The results are excerpted from ApolloScape leaderboard to make sure a fair comparison.
\begin{itemize}
    \setlength\itemsep{0.1em}
    \item StarNet\cite{zhu2019starnet}: The champion of \todo{trajectory prediction challenge at CVPR worksop}.\footnote{Need one or two sentences to summerize the results.}
    \item TrafficPredict\cite{ma2019trafficpredict}: An LSTM-based algorithm which focuses on predicting trajectories for heterogeneous traffic-agents in urban environment.
    \item LSTM: A simple LSTM encoder-decoder which only models each agent's temporal context independently.
    \item CV(constant velocity): A baseline which uses a constant velocity Kalman filter to predict trajectories in the future.
\end{itemize}
% All result are recorded from the public leaderboard.
In \autoref{tab:apollo}, the results show that our proposed method achieves best performance in every metric and every agent type.
Especially, compared with the current state-of-the-art method StarNet which is an LSTM-based attention network, we observe a \textbf{0.63m} improvement in FDE for vehicle prediction task.
Although they have leveraged a hub network with expensive computation on pairwise social interactions, the encoded context is still worse than ours.
Our method gets a considerable improvement compared with this LSTM-based spatio-temporal encoder on all three kind of traffic-agents.


\paragraph{Argoverse}
We compare our method with several baselines from Argoverse.
\begin{itemize}
    \item Nearest Neighbor with map (NN + map): Weighted Nearest Neighbor regression trajectories where trajectories are queried by coordinate in the curvilinear coordinate system.
    \item LSTM + map: standard LSTM encoder-decoder structure, which uses map information to define multiple curvilinear coordinate systems. Therefore, it can generate multiple possible future trajectories.
    \item LSTM + social + map : Similar to LSTM + map, but with additional hand-crafted social features. Social features include minimum distance to the vehicle in front and in back, and number of neighbors.
\end{itemize}

Table~\ref{tab:argo} \footnote{To be revised}shows that \pmethodb~outperforms all baselines on both $1s$ and $2s$ ADE metrics.
We also provide qualitative results to visualize how \pmethodb~can predict multiple possible future trajectories according to maps.

\begin{table}[!htbp]
    \centering
    % \scriptsize
    \begin{tabular*}{0.45\textwidth}{
                % >{\tiny}Ym{0.4in}
                >{}Ym{1.3in}
                >{}Ym{0.6in}<{\centering}  Ym{0.6in}<{\centering}
                % Ym{0.52in}<{\centering}  Ym{0.52in}<{\centering}
        }
        \toprule
        \rowstyle{}
        &\multicolumn{1}{c}{{$1s$ ADE}}  &\multicolumn{1}{c}{{$3s$ ADE}}  \\
        \midrule{}                                                                                                                 
        NN + map  &  0.72   &  2.28   \\ 
        LSTM + map  &  0.80   &  2.25 \\
        LSTM + social + map  &  0.89   &  2.46 \\ 
        \pmethodb~  &  /   &  \textbf{1.47}  \\ 
        \bottomrule
    \end{tabular*}
    \caption{Evaluations on the Argoverse dataset.}
\end{table}\label{tab:argo}


% \begin{figure}[!t]
%         \centerline{
%         \subfigure[\footnotesize{Clipping range}]{\includegraphics[width=0.245\textwidth]{figs/2d_representation.png} \label{fig_kl2clip_discrete_ratio}}
%         \subfigure[\footnotesize{Clipping range}]{\includegraphics[width=0.245\textwidth]{figs/2d_representation.png} \label{fig_kl2clip_discrete_probability}}
%         }
%             % \caption{
%             %     (a) 
%             %     (b) 
%             %     The hyperparameter of \pmethod is $\delta=0.02$, while that of PPO $\epsilon=0.2$.  
%             % }\label{fig_kl2clip_discrete}
%     \end{figure}
\begin{figure*}[!t]
        \centerline{
        \subfigure{\includegraphics[width=0.245\textwidth]{figs/argo_viz/0.pdf} \label{dd}}
        \subfigure{\includegraphics[width=0.245\textwidth]{figs/argo_viz/1.pdf} \label{dd}}
        \subfigure{\includegraphics[width=0.245\textwidth]{figs/argo_viz/2.pdf} \label{ss}}
        \subfigure{\includegraphics[width=0.245\textwidth]{figs/argo_viz/3.pdf} \label{ss}}
        }
        \centerline{
        \subfigure{\includegraphics[width=0.245\textwidth]{figs/argo_viz/4.pdf} \label{dd}}
        \subfigure{\includegraphics[width=0.245\textwidth]{figs/argo_viz/5.pdf} \label{dd}}
        \subfigure{\includegraphics[width=0.245\textwidth]{figs/argo_viz/6.pdf} \label{ss}}
        \subfigure{\includegraphics[width=0.245\textwidth]{figs/argo_viz/7.pdf} \label{ss}}
        }
        \caption{
            Validation of \pmethodb~ on Argoverse dataset.
        }\label{d}
\end{figure*}

\paragraph{NGSIM}
We report the performance of \pmethodb~and several state-of-the-art algorithms on the NGSIM dataset.
Only deterministic version result is reported.
In addition, we construct a variant of our method denoted as \textit{\pmethodb-180} which doubles the context range by enlarging the longitudinal direction range from $\pm 90$ to $\pm 180$.

Without any doubt, \pmethodb~outperforms any other algorithm in the same setting. In particular, the results of $\pm 180$ improves dramatically. It outperforms the standard version, especially in the result of $5s$.
We believe that it is owe to the richer spatio-temporal context provided, and our unified modeling method could digest these information seamlessly.


\begin{table*}[!htbp]
	\centering
		\begin{tabular}{@{}
			+m{0.6in}<{\centering}
			Ym{0.4in}<{\centering}Ym{0.4in}<{\centering}
			Ym{0.4in}<{\centering}Ym{0.4in}<{\centering}
			Ym{0.4in}<{\centering}Ym{0.4in}<{\centering}
            Ym{0.4in}<{\centering}Ym{0.4in}<{\centering}
			% @{}}            
			Ym{0.4in}<{\centering}Ym{0.4in}<{\centering}Ym{0.4in}<{\centering}
			Ym{0.4in}<{\centering}Ym{0.6in}<{\centering}Ym{0.4in}<{\centering}Ym{0.4in}<{\centering}
			@{}}
			\toprule
			% & \multicolumn{5}{c}{(a) Episodes to hit threshold } & \multicolumn{4}{c} {(b) Maximum Rewards}   \\
            \noalign{\smallskip}
            \rowstyle{\small} 
            Time   & CV & CVGMM & GAIL-GRU   & LSTM   & MATF\cite{zhao2019multi}  & CS-LSTM  &  S-LSTM  &\pmethodb~  & \pmethodb-180  \\
			\midrule{}
			%\multirow{8}{*}{$\epsilon=0.0$}										
			1$s$  &  0.73  &  0.66 & 0.69 & 0.68 & 0.67   & 0.61 & 0.65 & \textbf{0.58} & 0.56     \\ 
			2$s$  &  1.78  &  1.56 & 1.56 & 1.65 & 1.51   & 1.27 & 1.31 & \textbf{1.20} & 1.15     \\ 
			3$s$  &  3.13  &  2.75 & 2.75 & 2.91 & 2.51   & 2.09 & 2.16 & \textbf{1.96} & 1.82     \\ 
			4$s$  &  4.78  &  4.24 & 4.24 & 4.46 & 3.71   & 3.10 & 3.25 & \textbf{2.92} & 2.58     \\ 
			5$s$  &  6.68  &  5.99 & 5.99 & 6.27 & 5.12   & 4.37 & 4.55 & \textbf{4.12} & 3.45     \\ 
			\bottomrule
        \end{tabular}
        \caption{
	Result on NGSIM
	}\label{tab:ngsim}
\end{table*}

\subsection{Ablation Study}
In this section, we design several variants of \pmethodb~how different setting influent the final performance. All methods are evaluated on argoverse validation set.
\textbf{Input representation} we study the choice of the input representation in \pmethodb~. Table 3 shows the results of different input.
Note that the velocity comes from the position divided time interval. The results in Table 3 demonstrate that \pmethodb~.
As can be noticed, velocity does not bring great improvement after adding time to input. 
Thus, we believe that \pmethodb~ can model the relationship between different agents across spatio and temporal space.
  

\begin{table}[!htbp]
	\centering
		\begin{tabular}{@{}
			Ym{0.4in}<{\centering}Ym{0.4in}<{\centering}
			Ym{0.4in}<{\centering}Ym{0.4in}<{\centering}
			Ym{0.4in}<{\centering}Ym{0.4in}<{\centering}
            % Ym{0.4in}<{\centering}Ym{0.4in}<{\centering}
			% % @{}}            
			% Ym{0.4in}<{\centering}Ym{0.4in}<{\centering}Ym{0.4in}<{\centering}
			% Ym{0.4in}<{\centering}Ym{0.6in}<{\centering}Ym{0.4in}<{\centering}Ym{0.4in}<{\centering}
			@{}}
			\toprule
			% & \multicolumn{5}{c}{(a) Episodes to hit threshold } & \multicolumn{4}{c} {(b) Maximum Rewards}   \\
            \noalign{\smallskip}
            \rowstyle{\small} 
            pos &  time &  vel   &    ADE  & FDE \\ 
			\midrule{}
			%\multirow{8}{*}{$\epsilon=0.0$}										
			\checkmark  &             &             &  3.384  & 6.893  \\ 
			\checkmark  &  \checkmark &             &  2.131  & 3.7098 \\ 
			\checkmark  &  \checkmark &  \checkmark &  2.019  & 3.2907 \\ 
			\bottomrule
        \end{tabular}
        \caption{
	Results on the Argoverse validation set.
	}\label{tab:ablation}
\end{table}

\textbf{Number of Refinement blocks} We also conduct ablation study to explore how many refinement blocks are needed for \pmethodb~. 
The results in Table 4 shows that when the number of refinement blocks beyound 2, the performance
of \pmethodb~ becomes stable. This movtivate \pmethodb~ to be designed as a fast and light network.

\begin{figure}[!htbp]
	\centering
	\includegraphics[width=0.44\textwidth]{figs/number_refine_blocks.pdf}
	\caption[width=\columnwidth]{
		Results on the Argoverse val set using different number of refinement blocks
   }\label{fig:number_refine_blocks}
\end{figure}


\begin{figure*}[!t]
    \centerline{
    \subfigure{\includegraphics[width=0.2\textwidth]{figs/ablation/pattern_b/pattern_229.png} \label{dd}}
    \subfigure{\includegraphics[width=0.2\textwidth]{figs/ablation/pattern_b/8.61.png} \label{dd}}
    \subfigure{\includegraphics[width=0.2\textwidth]{figs/ablation/pattern_b/5.87.png} \label{dd}}
    \subfigure{\includegraphics[width=0.2\textwidth]{figs/ablation/pattern_b/1.48.png} \label{dd}}
    \subfigure{\includegraphics[width=0.2\textwidth]{figs/ablation/pattern_b/0.19.png} \label{dd}}
    }
    \centerline{
        \subfigure{\includegraphics[width=0.2\textwidth]{figs/ablation/pattern_a/pattern_65.png} \label{dd}}
        \subfigure{\includegraphics[width=0.2\textwidth]{figs/ablation/pattern_a/8.62.png} \label{dd}}
        \subfigure{\includegraphics[width=0.2\textwidth]{figs/ablation/pattern_a/6.21.png} \label{dd}}
        \subfigure{\includegraphics[width=0.2\textwidth]{figs/ablation/pattern_a/2.34.png} \label{dd}}
        \subfigure{\includegraphics[width=0.2\textwidth]{figs/ablation/pattern_a/0.38.png} \label{dd}}
    }
    \caption{
        Validation of \pmethodb~ on Argoverse dataset.
    }\label{fig:partition}
\end{figure*}
